Inter-sensor propagation delay estimation using sources of opportunity

Propagation delays are intensively used for Structural Health Monitoring or Sensor Network Localization. In this paper, we study the performances of acoustic propagation delay estimation between two sensors, using sources of opportunity only. Such sources are defined as being uncontrolled by the user (activation time, location, spectral content in time and space), thus preventing the direct estimation with classical active approaches, such as TDOA, RSSI and AOA. Observation models are extended from the literature to account for the spectral characteristics of the sources in this passive context and we show how time-filtered sources of opportunity impact the retrieval of the propagation delay between two sensors. A geometrical analogy is then proposed that leads to a lower bound on the variance of the propagation delay estimation that accounts for both the temporal and the spatial properties of the sources field.

==> part4.tex <==
\subsection{A lower bound for passive minimum propagation delay estimation}

Equation \eqref{m:cgest2} in section \ref{ss:model} provides the observation model
\begin{equation}
\mb{gc}[n] = \int_0^{2\pi} p_\theta(\theta) \gamma_s( \mb{t}[n] - \tau\cos(\theta)) d\theta + \mb{w}[n].
\label{m:rgf}
\end{equation}

In Equation \eqref{m:rgf}, $\mb{gc}[n]$ is the retrieved Green's correlation function at time $n$. $\mb{t}$ is the time vector of length $N$. $\mb{w}$ is the noise in the model. It is formed from the estimations of the auto-correlation function of the sources and their average. In the light of the previous results, $\mb{w}$ is a i.i.d. zero-mean Gaussian sequence, with variance $\boldsymbol\sigma^2[n]$. The Fisher information on the minimum propagation delay $\tau$ writes
\begin{equation}
F_\tau(\mb{t},p_\theta) = \frac{1}{\boldsymbol\sigma^2} \Big[ \int_0^{2\pi} p_\theta(\theta) \cos(\theta) \frac{\partial \gamma_s}{\partial t} ( \mb{t} - \tau\cos(\theta)) d\theta \Big]^2.
\label{m:fisher2}
\end{equation}


Assume that the variance of the noise can be approximated constant, $\boldsymbol\sigma[n]^2 = \sigma^2$. Denote $E$ the energy of the retrieved Green's correlation,
\begin{equation*}
E = \sum_{i=1}^N \Big( \int_{0}^{2\pi} p_\theta(\theta) \gamma_s( \mb{t}[n]-\tau\cos(\theta) ) d\theta \Big)^2
\label{m:energy}
\end{equation*}
and denote $\bar\beta^2$ the normalized angular bandwidth, see \cite{Ziv},
\begin{equation*}
\bar\beta^2 = \frac{1}{E}\sum_{i=1}^N \Big( \frac{\partial}{\partial t}\int_0^{2\pi} p_\theta(\theta) \cos(\theta) \gamma_s( \mb{t}[n] - \tau\cos(\theta)) d\theta \Big)^2.
\label{m:beta}
\end{equation*}

The Fisher information then takes a classical form, see for instance \cite{Ziv,Kay1993},
\begin{equation}
F_\tau(p_\theta) = \frac{ E }{\sigma^2} \times \bar\beta^2.
\label{m:fishertotal}
\end{equation}

From Equation \eqref{m:fishertotal}, a Cramer-Rao lower bound for the passive estimation of parameters can be derived. Using Cauchy-Schwartz, see \textit{e.g.} \cite{Kay1993} or the Chebychev inequality, see \textit{e.g.} \cite{Ziv}, it can be shown that the mean square error on the passive propagation delay estimation is bounded by
\begin{equation}
mse \geq \frac{1}{F_\tau(p_\theta)},
\label{m:msebound1}
\end{equation}

\subsubsection{Examples of analytical p-CRB} 

\rv{}{
Applying this result to study case (1), Fig. \ref{f:unifcv}, then $mse \geq \pi \sigma^2 / 2N$. In comparison, study case (3) in Fig. \ref{f:uniffilt} presents a bias, which leads to $mse \geq \frac{1 }{1/4 + 0.168 N / \pi \sigma^2 }$. Note a model for the Green's correlation in a bounded medium would allow to evaluate the passive Cramer-Rao lower bound in practical cases.
}

\subsubsection{p-CRB in an experimental context} 

\rv{}{Exemples d'applications de la borne :}

\begin{itemize}
	\item \rv{}{Modèle d'observation de la corrélation de Green : à partir du bruit de mesure (variance $e-8~V^2$), signaux d'amplitude $20mV$, bande 44kHz, hypothèse d'uniformité spatiale, taille de la corrélation N échantillons; il faut identifier la variance du bruit sur la corrélation de Green pour pouvoir calculer la p-CRB. Deux approches possibles :}
	\begin{itemize}
		\item on dispose d'un modèle de la corrélation de Green, auquel cas on peut estimer la variance du bruit de modèle;
		\item on donne un ordre de grandeur, associé aux opérations qui sont impiquées dans l'estimation de la corrélation de Green. Cumul de 1300 estimations de la corrélation de Green, réalisées à partir de N échantillons et donc souffrant d'un bruit de variance v. Attention, ici le moyennage d'ensemble (spatial) n'est pas intégré dans la chaîne de modélisation du bruit; on fait l'hypothèse que la diversité spatiale est "complète" sur chaque fenêtre.
	\end{itemize}
	\item \rv{}{Modèle d'observation sur la fonction de Green : on recherche un pulse, noyé dans du bruit. La variance du bruit est déjà estimée dans la table I. Le calcul de la borne est direct. Attention, le modèle d'observation n'a plus rien d'original.}
\end{itemize} 

%Expression \eqref{m:msebound1} displays the influence of the distribution $p_\theta$ of the incidence angles. It is however hard to interpret further. In the following, the notion of information will be depicted from the incidence direction, for one source.
%
%%\begin{eg}
%%
%%Consider the following assumptions:
%%\begin{itemize}
%%	\item incidence angles are i.i.d. uniform variables in $[0,2\pi]$;
%%	\item the sources are white i.i.d random process;
%%	\item the variance of the noise in the model \eqref{m:rgf} is constant
%%	\item sampling period is $\Delta$
%%\end{itemize}
%%then the Fisher information writes:
%%\begin{equation}
%%F_\tau = \frac{(N\Delta)^3}{\pi^2\sigma^2\tau^2} \Big[ \mathrm{atanh}{ \Big( \frac{N\Delta}{\tau} \Big)} - \frac{4}{3}\Big( \frac{N\Delta}{\tau}\Big)^3 \Big]
%%\label{m:ex_fisher}
%%\end{equation}
%%
%%\end{eg}
%
%\subsection{Interpretations}
%
%An analogy is proposed, simply to better grasp the notion of spatial information induced by various incidence direction. Each source are treated separately and a new propagation delay estimator is proposed for the occasion.
%
%In the source-sensor setup from Fig. \ref{f:anglearrival}, one source impiges on the sensor set with an incidence angle $\theta$.
%
%Using one source only, the matched filter allows to estimate the path delay difference. 
%
%Recall that the Cramèr-Rao bound is of the form:
%\begin{equation}
%\sigma_{crlb}^2(\tau) =  \frac{1}{\mathrm{SNR} \times \bar{F}^2}
%\label{m:crlba}
%\end{equation}
%where $\mathrm{SNR}$ is the signal-to-noise ratio and $\bar{F}$ measures the bandwidth of the source signal.
%
%However, we here tackle the estimation of the inter-sensor propagation delay, from a set of path delay differences that were estimated with no bias and variance $\sigma^2_{crlb}$. The observation model is:
%\begin{equation}
%\mb{t} = \tau \cos(\boldsymbol\theta) + \mb{w}
%\label{m:mesure}
%\end{equation}
%where $\tau$ is the parameter to estimate, seen through measurements $\mb{t}$ that are composed of biased versions of the parameter, corrupted by $\mb{w}$, a zero-mean normal random variable, with variance $\sigma^2_{crlb}$.
%In this case, the problem is equivalent to an amplitude estimation problem. 
%
%One source carries the Fisher information $F_\tau(\theta)$:
%\begin{equation}
%F_\tau(\theta) = \frac{\cos^2{\theta}}{\sigma^2_{crlb}}.
%\label{m:onesourceinfo}
%\end{equation}
%where it is clear the information carried by a source changes with its incidence angle; when the incidence vector $\vec{k}$ statisfies $\langle \vec{x}-\vec{y},\vec{k}(\theta) \rangle = 0$, the path-delay difference is null and so is the information. On the other hand, the variance tends to its minimum $\sigma_{crlb}^2$ as the source and the sensor array are aligned. Also, Equation \eqref{m:onesourceinfo} allows symmetries and invariances to be identified as $\cos^2(\theta) = \cos^2(\pi-\theta) = \cos^2(-\theta)$, which allows $\theta$ to be picked in $[0;\pi/2]$ only. 
%
%For all source, the total Fisher information can be found in \cite{Kay1993} and writes:
%\begin{equation}
%F_\tau = \frac{1}{\sigma^2} \sum_{i=0}^{N-1} \cos^2(\theta)
%\label{m:fisher1}
%\end{equation}
%
%For N large enough, one has:
%\begin{equation}
%mse \geq \frac{2\sigma^2 (1 + B'(\tau))}{N} + B^2(\tau)
%\label{m:fisher_opt}
%\end{equation}
%
%where the bias depends on the distribution
%
%Given the observation model \eqref{m:mesure}, the proposed propagation delay estimator is derived from the energy estimator:
%\begin{equation}
%\hat\tau = \sqrt{2 \hat E}\textrm{, with }\hat E = \frac{1}{N} \sum_{i=0}^{N-1} \mb{t}^2[n].
%\label{m:energyest}
%\end{equation}
%
%
%$\hat E$ has bias $\sigma^2_{crlb}$ and variance $\sigma^2 = \frac{1}{N}(\sigma^2_{crlb} \tau^2)$.
%
%using tbeghjdgkjn it can be shown that $\hat \tau$ then has bias $pouet$ and variance $pouet$.
